Chemo-dynamical stratification of the Galactic disc using \emph{Gaia}-ESO open clusters

Understanding how the Milky Way disc assembled and evolved requires tracing the coupled evolution of stellar chemistry and orbital structure over time. Open clusters, as coeval stellar populations with well-constrained ages, distances, and chemical properties, provide powerful benchmarks for this purpose. We aim to characterise the age-dependent chemo-dynamical structure of the Galactic disc and to investigate how open clusters populate dynamical phase space as a function of age. We analysed a sample of Galactic open clusters using homogeneous chemical abundances from the Gaia-ESO Survey together with Gaia DR3 phase-space information. Combining cluster ages with orbital parameters and actions, we examined how clusters populate dynamical phase space over the last ~4 Gyr. We find that clusters with similar chemical properties occupy coherent regions of action space, while their orbital structure shows a clear dependence on age. Radial excursions and orbital eccentricities broaden systematically toward older ages, indicating increasingly diverse orbital configurations in the older cluster population. The dispersion in the [Fe/H]-Rg relation also increases with age, consistent with a combination of secular redistribution, survival bias, and dynamically distinct outer-disc populations. In addition, older clusters reach larger vertical amplitudes and vertical actions, revealing a coupled but anisotropic evolution between in-plane and vertical orbital structure. Open clusters provide precise, age-resolved tracers of the chemo-dynamical structure of the Galactic disc. Our results reveal systematic age-dependent variations in the orbital and chemical properties of the cluster population, consistent with the combined effects of secular evolution, orbital redistribution, and environmentally dependent cluster survival over the last few Gyr.

==> image/table_orbital_parameters_science.tex <==
\begin{longtable}{lcccccccccccccccccccccc}
\caption{Derived orbital parameters for the SCIENCE sample of Gaia--ESO open clusters. Columns give heliocentric distance ($d$; pc), age (Gyr), pericentre and apocentre radii (kpc), orbital eccentricity, maximum vertical excursion (kpc), orbital actions ($J_R$, $J_{\phi}$, $J_Z$; kpc\,km\,s$^{-1}$), and guiding radius (kpc). Uncertainties are 1$\sigma$.} \label{tab:orbital_parameters_science} \\
\toprule
GES\_FLD &
$d$ &
$\sigma_d$ &
$\log\,\mathrm{Age}$ &
$\sigma_{\log\mathrm{Age}}$ &
$\mathrm{Age}$ &
$\sigma_{\mathrm{Age}}$ &
$R_{\mathrm{peri}}$ &
$\sigma_{R_{\mathrm{peri}}}$ &
$R_{\mathrm{apo}}$ &
$\sigma_{R_{\mathrm{apo}}}$ &
$e$ &
$\sigma_e$ &
$Z_{\max}$ &
$\sigma_{Z_{\max}}$ &
$J_R$ &
$\sigma_{J_R}$ &
$J_{\phi}$ &
$\sigma_{J_{\phi}}$ &
$J_Z$ &
$\sigma_{J_Z}$ &
$R_g$ &
$\sigma_{R_g}$ \\
\midrule
 &
(pc) &
(pc) &
(-) &
(-) &
(Gyr) &
(Gyr) &
(kpc) &
(kpc) &
(kpc) &
(kpc) &
(–) &
(–) &
(kpc) &
(kpc) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc) &
(kpc) \\
\midrule
\endfirsthead
\caption[]{Derived orbital parameters for the SCIENCE sample of Gaia--ESO open clusters. Columns give heliocentric distance ($d$; pc), age (Gyr), pericentre and apocentre radii (kpc), orbital eccentricity, maximum vertical excursion (kpc), orbital actions ($J_R$, $J_{\phi}$, $J_Z$; kpc\,km\,s$^{-1}$), and guiding radius (kpc). Uncertainties are 1$\sigma$. Values are truncated to three decimal places.} \\
\toprule
GES\_FLD &
$d$ &
$\sigma_d$ &
$\log\,\mathrm{Age}$ &
$\sigma_{\log\mathrm{Age}}$ &
$\mathrm{Age}$ &
$\sigma_{\mathrm{Age}}$ &
$R_{\mathrm{peri}}$ &
$\sigma_{R_{\mathrm{peri}}}$ &
$R_{\mathrm{apo}}$ &
$\sigma_{R_{\mathrm{apo}}}$ &
$e$ &
$\sigma_e$ &
$Z_{\max}$ &
$\sigma_{Z_{\max}}$ &
$J_R$ &
$\sigma_{J_R}$ &
$J_{\phi}$ &
$\sigma_{J_{\phi}}$ &
$J_Z$ &
$\sigma_{J_Z}$ &
$R_g$ &
$\sigma_{R_g}$ \\

\midrule
\endhead
\midrule
\multicolumn{23}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Blanco1 & 234.390 & 0.094 & 8.239 & 0.309 & 0.173 & 0.140 & 8.079 & 0.004 & 8.713 & 0.001 & 0.037 & 0.000 & 0.215 & 0.001 & 1.867 & 0.021 & 1938.128 & 0.520 & 1.551 & 0.019 & 8.371 & 0.002 \\
Br21 & 5294.645 & 152.808 & 8.945 & 0.255 & 0.881 & 0.606 & 12.240 & 0.135 & 14.211 & 0.215 & 0.074 & 0.010 & 0.235 & 0.007 & 10.722 & 2.986 & 2888.963 & 21.462 & 0.949 & 0.041 & 13.157 & 0.111 \\
Br22 & 5334.363 & 128.064 & 8.897 & 0.263 & 0.789 & 0.545 & 10.910 & 0.257 & 14.559 & 0.221 & 0.143 & 0.017 & 0.789 & 0.020 & 38.060 & 9.047 & 2749.343 & 25.489 & 7.940 & 0.281 & 12.436 & 0.131 \\
Br30 & 4462.350 & 73.578 & 8.663 & 0.180 & 0.460 & 0.190 & 11.439 & 0.114 & 12.697 & 0.469 & 0.050 & 0.019 & 0.278 & 0.007 & 4.426 & 4.838 & 2672.182 & 40.891 & 1.518 & 0.030 & 12.039 & 0.209 \\
Br31 & 5864.814 & 174.234 & 9.075 & 0.228 & 1.190 & 0.708 & 10.954 & 0.180 & 13.708 & 0.174 & 0.111 & 0.007 & 0.587 & 0.015 & 22.195 & 3.176 & 2693.462 & 29.961 & 5.216 & 0.146 & 12.148 & 0.153 \\
Br32 & 3147.859 & 21.970 & 9.512 & 0.150 & 3.252 & 1.213 & 7.219 & 0.086 & 11.831 & 0.057 & 0.242 & 0.007 & 0.289 & 0.002 & 85.394 & 5.436 & 2069.601 & 9.988 & 1.771 & 0.020 & 9.010 & 0.048 \\
Br36 & 3839.619 & 48.311 & 9.018 & 0.182 & 1.042 & 0.443 & 11.048 & 0.050 & 11.370 & 0.139 & 0.014 & 0.005 & 0.258 & 0.008 & 0.343 & 0.295 & 2506.479 & 16.260 & 1.545 & 0.077 & 11.193 & 0.082 \\
Br39 & 3809.337 & 30.210 & 9.494 & 0.149 & 3.125 & 1.133 & 8.245 & 0.027 & 11.363 & 0.031 & 0.158 & 0.001 & 0.999 & 0.016 & 37.032 & 0.484 & 2158.078 & 5.148 & 16.377 & 0.339 & 9.445 & 0.025 \\
Br44 & 2690.292 & 20.772 & 9.003 & 0.182 & 1.008 & 0.470 & 5.511 & 0.122 & 7.376 & 0.019 & 0.144 & 0.009 & 0.223 & 0.002 & 21.829 & 2.695 & 1493.761 & 19.283 & 2.038 & 0.044 & 6.306 & 0.085 \\
Br73 & 6497.806 & 279.208 & 9.128 & 0.176 & 1.343 & 0.562 & 13.314 & 0.380 & 15.805 & 0.440 & 0.086 & 0.006 & 1.304 & 0.085 & 15.779 & 2.348 & 3111.288 & 74.399 & 17.148 & 1.319 & 14.315 & 0.389 \\
Br75 & 6829.598 & 290.963 & 9.269 & 0.205 & 1.858 & 0.996 & 9.710 & 0.391 & 13.464 & 0.237 & 0.162 & 0.011 & 1.326 & 0.051 & 44.743 & 5.267 & 2496.357 & 65.916 & 21.093 & 0.989 & 11.141 & 0.334 \\
Br81 & 3468.979 & 46.229 & 8.352 & 0.207 & 0.225 & 0.112 & 5.535 & 0.063 & 6.293 & 0.087 & 0.064 & 0.003 & 0.159 & 0.002 & 4.108 & 0.453 & 1397.674 & 16.580 & 1.289 & 0.043 & 5.883 & 0.072 \\
Col197 & 924.127 & 1.751 & 6.605 & 0.109 & 0.004 & 0.000 & 8.204 & 0.251 & 8.447 & 0.207 & 0.021 & 0.013 & 0.043 & 0.001 & 0.584 & 1.206 & 1928.107 & 43.010 & 0.068 & 0.001 & 8.323 & 0.206 \\
Cz24 & 3722.727 & 90.968 & 9.080 & 0.180 & 1.203 & 0.502 & 9.280 & 0.027 & 11.969 & 0.117 & 0.126 & 0.005 & 0.346 & 0.019 & 25.298 & 2.297 & 2360.600 & 8.570 & 2.440 & 0.224 & 10.455 & 0.043 \\
Cz30 & 6108.557 & 169.368 & 9.033 & 0.189 & 1.081 & 0.487 & 10.157 & 0.145 & 13.328 & 0.173 & 0.135 & 0.001 & 0.493 & 0.015 & 31.485 & 0.724 & 2570.502 & 30.757 & 3.940 & 0.153 & 11.519 & 0.156 \\
ESO92\_05 & 11149.450 & 574.221 & 9.199 & 0.338 & 1.584 & 1.412 & 9.984 & 0.676 & 16.133 & 3.108 & 0.237 & 0.065 & 1.932 & 0.302 & 105.846 & 99.093 & 2693.215 & 242.282 & 30.886 & 2.077 & 12.147 & 1.243 \\
IC4665 & 343.345 & 0.239 & 7.514 & 0.230 & 0.032 & 0.017 & 7.383 & 0.089 & 7.922 & 0.007 & 0.035 & 0.006 & 0.129 & 0.002 & 1.464 & 0.529 & 1784.086 & 10.425 & 0.654 & 0.026 & 7.637 & 0.049 \\
M67 & 837.267 & 0.628 & 9.227 & 0.178 & 1.688 & 0.737 & 7.789 & 0.010 & 9.295 & 0.002 & 0.088 & 0.000 & 0.560 & 0.001 & 10.115 & 0.181 & 1946.596 & 1.085 & 8.009 & 0.037 & 8.412 & 0.005 \\
NGC2141 & 4052.221 & 34.795 & 9.262 & 0.154 & 1.831 & 0.707 & 11.710 & 0.046 & 12.967 & 0.096 & 0.050 & 0.005 & 0.410 & 0.004 & 4.671 & 0.963 & 2720.446 & 7.263 & 3.003 & 0.046 & 12.287 & 0.037 \\
NGC2158 & 3706.334 & 20.611 & 9.269 & 0.160 & 1.858 & 0.704 & 10.799 & 0.026 & 11.932 & 0.025 & 0.049 & 0.001 & 0.325 & 0.004 & 4.111 & 0.316 & 2531.236 & 2.864 & 2.213 & 0.046 & 11.319 & 0.014 \\
NGC2232 & 318.036 & 0.224 & 7.123 & 0.234 & 0.013 & 0.007 & 8.437 & 0.029 & 8.616 & 0.031 & 0.011 & 0.001 & 0.045 & 0.002 & 0.160 & 0.043 & 1969.963 & 5.964 & 0.073 & 0.006 & 8.525 & 0.028 \\
NGC2243 & 3928.227 & 23.567 & 9.439 & 0.167 & 2.748 & 1.115 & 10.445 & 0.019 & 16.863 & 0.124 & 0.234 & 0.002 & 1.838 & 0.022 & 109.860 & 2.952 & 2815.872 & 10.129 & 26.733 & 0.271 & 12.779 & 0.052 \\
NGC2244 & 1415.235 & 4.221 & 6.613 & 0.122 & 0.004 & 0.001 & 9.451 & 0.129 & 10.393 & 0.238 & 0.050 & 0.010 & 0.060 & 0.003 & 3.727 & 2.122 & 2251.631 & 30.092 & 0.103 & 0.014 & 9.910 & 0.150 \\
NGC2264 & 706.459 & 1.968 & 6.756 & 0.157 & 0.005 & 0.002 & 8.652 & 0.186 & 8.950 & 0.199 & 0.020 & 0.016 & 0.085 & 0.004 & 0.590 & 1.664 & 2023.196 & 26.543 & 0.253 & 0.019 & 8.783 & 0.129 \\
NGC2355 & 1751.095 & 5.018 & 9.232 & 0.171 & 1.706 & 0.674 & 9.754 & 0.110 & 10.906 & 0.176 & 0.057 & 0.007 & 0.599 & 0.033 & 5.286 & 1.676 & 2316.546 & 22.900 & 7.534 & 0.504 & 10.234 & 0.114 \\
NGC2420 & 2311.418 & 8.766 & 9.352 & 0.169 & 2.250 & 0.908 & 8.222 & 0.074 & 11.303 & 0.062 & 0.157 & 0.007 & 0.918 & 0.010 & 36.508 & 3.306 & 2153.989 & 5.499 & 14.210 & 0.151 & 9.425 & 0.027 \\
NGC2425 & 3094.027 & 21.859 & 9.295 & 0.160 & 1.975 & 0.729 & 8.202 & 0.050 & 11.593 & 0.032 & 0.171 & 0.002 & 0.490 & 0.008 & 43.723 & 1.177 & 2188.967 & 8.245 & 4.731 & 0.118 & 9.598 & 0.040 \\
NGC2451 & 367.535 & 0.148 & 7.440 & 0.223 & 0.027 & 0.015 & 8.305 & 0.001 & 8.857 & 0.094 & 0.032 & 0.005 & 0.063 & 0.001 & 1.369 & 0.464 & 1979.672 & 9.097 & 0.140 & 0.008 & 8.572 & 0.044 \\
NGC2516 & 407.088 & 0.089 & 8.097 & 0.269 & 0.125 & 0.089 & 7.310 & 0.021 & 8.183 & 0.000 & 0.056 & 0.001 & 0.095 & 0.000 & 3.861 & 0.198 & 1801.942 & 2.523 & 0.344 & 0.003 & 7.721 & 0.011 \\
NGC2547 & 382.382 & 0.179 & 7.336 & 0.259 & 0.021 & 0.014 & 8.190 & 0.011 & 8.764 & 0.127 & 0.033 & 0.006 & 0.053 & 0.002 & 1.501 & 0.626 & 1958.170 & 13.602 & 0.100 & 0.010 & 8.468 & 0.065 \\
NGC3532 & 471.884 & 0.109 & 8.376 & 0.249 & 0.237 & 0.155 & 7.988 & 0.020 & 8.062 & 0.001 & 0.004 & 0.001 & 0.121 & 0.000 & 0.025 & 0.014 & 1864.877 & 2.262 & 0.566 & 0.002 & 8.020 & 0.010 \\
NGC4815 & 3142.276 & 12.634 & 8.411 & 0.174 & 0.258 & 0.109 & 6.558 & 0.112 & 7.118 & 0.033 & 0.040 & 0.006 & 0.103 & 0.000 & 1.840 & 0.609 & 1608.696 & 16.518 & 0.480 & 0.007 & 6.824 & 0.075 \\
NGC6005 & 2388.113 & 9.511 & 8.933 & 0.171 & 0.857 & 0.339 & 4.935 & 0.070 & 6.374 & 0.007 & 0.127 & 0.007 & 0.115 & 0.000 & 15.206 & 1.619 & 1324.177 & 10.244 & 0.671 & 0.008 & 5.567 & 0.043 \\
NGC6067 & 1957.161 & 3.378 & 7.949 & 0.187 & 0.088 & 0.040 & 6.580 & 0.011 & 6.901 & 0.106 & 0.023 & 0.007 & 0.070 & 0.001 & 0.608 & 0.469 & 1589.522 & 10.960 & 0.236 & 0.005 & 6.737 & 0.049 \\
NGC6253 & 1606.201 & 3.190 & 9.267 & 0.167 & 1.852 & 0.779 & 5.335 & 0.016 & 6.849 & 0.007 & 0.124 & 0.000 & 0.216 & 0.001 & 15.333 & 0.222 & 1422.510 & 2.967 & 2.091 & 0.018 & 5.992 & 0.012 \\
NGC6259 & 2158.990 & 3.723 & 8.215 & 0.178 & 0.164 & 0.070 & 5.721 & 0.020 & 6.227 & 0.020 & 0.042 & 0.000 & 0.041 & 0.000 & 1.780 & 0.051 & 1416.017 & 4.592 & 0.090 & 0.001 & 5.963 & 0.020 \\
NGC6281 & 520.762 & 0.338 & 8.437 & 0.234 & 0.273 & 0.161 & 7.574 & 0.013 & 7.921 & 0.006 & 0.022 & 0.001 & 0.072 & 0.000 & 0.605 & 0.068 & 1806.311 & 0.859 & 0.207 & 0.001 & 7.742 & 0.004 \\
NGC6405 & 451.869 & 0.274 & 7.719 & 0.240 & 0.052 & 0.030 & 7.700 & 0.018 & 7.759 & 0.015 & 0.003 & 0.002 & 0.043 & 0.000 & 0.017 & 0.033 & 1803.377 & 0.657 & 0.077 & 0.001 & 7.728 & 0.003 \\
NGC6633 & 389.528 & 0.201 & 8.674 & 0.212 & 0.472 & 0.248 & 7.212 & 0.034 & 8.133 & 0.004 & 0.060 & 0.002 & 0.082 & 0.000 & 4.348 & 0.379 & 1785.875 & 3.570 & 0.260 & 0.000 & 7.646 & 0.016 \\
NGC6709 & 1048.055 & 1.571 & 8.207 & 0.210 & 0.161 & 0.088 & 7.030 & 0.155 & 7.561 & 0.009 & 0.036 & 0.011 & 0.146 & 0.002 & 1.515 & 1.030 & 1707.541 & 17.164 & 0.882 & 0.027 & 7.279 & 0.079 \\
NGC6802 & 2768.780 & 13.561 & 8.534 & 0.175 & 0.342 & 0.145 & 6.305 & 0.132 & 7.450 & 0.133 & 0.084 & 0.003 & 0.067 & 0.000 & 7.856 & 0.639 & 1610.858 & 29.043 & 0.193 & 0.001 & 6.834 & 0.132 \\
Pismis15 & 2254.343 & 10.105 & 8.652 & 0.182 & 0.448 & 0.201 & 7.215 & 0.159 & 8.421 & 0.005 & 0.077 & 0.010 & 0.140 & 0.000 & 7.289 & 1.983 & 1812.396 & 19.757 & 0.708 & 0.007 & 7.771 & 0.093 \\
Pismis18 & 2598.111 & 12.083 & 8.508 & 0.184 & 0.322 & 0.154 & 6.502 & 0.036 & 6.919 & 0.004 & 0.031 & 0.002 & 0.090 & 0.000 & 1.037 & 0.181 & 1581.745 & 4.387 & 0.385 & 0.007 & 6.701 & 0.019 \\
Rup134 & 2296.640 & 12.284 & 8.308 & 0.218 & 0.203 & 0.104 & 4.534 & 0.093 & 6.241 & 0.160 & 0.158 & 0.022 & 0.109 & 0.005 & 22.591 & 6.904 & 1252.751 & 3.717 & 0.631 & 0.038 & 5.265 & 0.015 \\
Trumpler14 & 2296.983 & 6.845 & 6.794 & 0.208 & 0.006 & 0.003 & 7.789 & 0.509 & 7.832 & 0.630 & 0.043 & 0.036 & 0.030 & 0.001 & 2.325 & 6.472 & 1820.377 & 102.753 & 0.037 & 0.005 & 7.809 & 0.486 \\
Trumpler20 & 3279.385 & 10.675 & 9.200 & 0.163 & 1.584 & 0.592 & 7.014 & 0.002 & 7.750 & 0.028 & 0.049 & 0.001 & 0.162 & 0.000 & 2.923 & 0.209 & 1724.141 & 3.025 & 1.040 & 0.005 & 7.356 & 0.014 \\
Trumpler23 & 2471.292 & 10.055 & 8.520 & 0.164 & 0.331 & 0.123 & 5.042 & 0.091 & 6.399 & 0.065 & 0.118 & 0.004 & 0.018 & 0.000 & 13.424 & 0.842 & 1343.303 & 19.057 & 0.017 & 0.001 & 5.649 & 0.081 \\
Trumpler5 & 2904.927 & 9.492 & 9.337 & 0.166 & 2.173 & 0.850 & 10.702 & 0.019 & 12.289 & 0.014 & 0.069 & 0.000 & 0.104 & 0.000 & 8.113 & 0.182 & 2556.112 & 2.946 & 0.242 & 0.001 & 11.445 & 0.015 \\
gamma2\_Vel & 346.884 & 0.166 & 6.971 & 0.225 & 0.009 & 0.004 & 8.248 & 0.074 & 8.338 & 0.140 & 0.008 & 0.007 & 0.067 & 0.004 & 0.088 & 0.307 & 1921.525 & 18.842 & 0.169 & 0.019 & 8.291 & 0.090 \\
lam\_Ori & 393.775 & 0.213 & 6.719 & 0.157 & 0.005 & 0.001 & 8.527 & 0.037 & 8.948 & 0.011 & 0.023 & 0.002 & 0.071 & 0.003 & 0.774 & 0.155 & 2012.117 & 4.313 & 0.175 & 0.017 & 8.729 & 0.020 \\
\end{longtable}

==> table_clusters_longB.tex <==
\begin{longtable}{lcccccccccccccccccc}
\caption{Summary properties of the final sample of 59 Gaia--ESO open clusters. Columns give mean coordinates, sample sizes, kinematics, chemistry, Gaia DR3 astrometry, distance, and age. Values are truncated to three decimal places. Superscripts indicate sample membership: $^{\mathrm{G}}$ (GOLD) and $^{\mathrm{S}}$ (SCIENCE).}\\
\toprule
ID &
RA &
Dec &
$N_{\rm obs}$ &
$N_{\rm mem}$ &
$\mathrm{SNR}_{\rm med}$ &
$\mathrm{RV}_{\rm mean}$ &
$\mathrm{RV}_{\rm std}$ &
$\mathrm{[Fe/H]}$ &
$\sigma_{\mathrm{[Fe/H]}}$ &
$A(\mathrm{Mg})$&
$\sigma_{A(\mathrm{Mg})}$ &
$\mu_{\alpha*}$ &
$\sigma_{\mu_{\alpha*}}$ &
$\mu_{\delta}$ &
$\sigma_{\mu_{\delta}}$ &
$\varpi$ &
$d$ &
$\log(\mathrm{Age})$ \\
\midrule
 &
(deg) &
(deg) &
(–) &
(–) &
(–) &
(km\,s$^{-1}$) &
(km\,s$^{-1}$) &
(dex) &
(dex) &
(dex) &
(dex) &
(mas\,yr$^{-1}$) &
(mas\,yr$^{-1}$) &
(mas\,yr$^{-1}$) &
(mas\,yr$^{-1}$) &
(mas) &
(pc) &
(dex) \\
\midrule
\endfirsthead

\toprule
ID &
RA &
Dec &
$N_{\rm obs}$ &
$N_{\rm mem}$ &
$\mathrm{SNR}_{\rm med}$ &
$\mathrm{RV}_{\rm mean}$ &
$\mathrm{RV}_{\rm std}$ &
$\mathrm{[Fe/H]}$ &
$\sigma_{\mathrm{[Fe/H]}}$ &
$A(\mathrm{Mg})$&
$\sigma_{A(\mathrm{Mg})}$ &
$\mu_{\alpha*}$ &
$\sigma_{\mu_{\alpha*}}$ &
$\mu_{\delta}$ &
$\sigma_{\mu_{\delta}}$ &
$\varpi$ &
$d$ &
$\log(\mathrm{Age})$ \\
\midrule
 &
(deg) &
(deg) &
(–) &
(–) &
(–) &
(km\,s$^{-1}$) &
(km\,s$^{-1}$) &
(dex) &
(dex) &
(dex) &
(dex) &
(mas\,yr$^{-1}$) &
(mas\,yr$^{-1}$) &
(mas\,yr$^{-1}$) &
(mas\,yr$^{-1}$) &
(mas) &
(pc) &
(dex) \\
\midrule
\endhead

\midrule
\multicolumn{19}{r}{Continued on next page} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
Blanco1$^{\mathrm{SG}}$ & 0.914 & -30.010 & 21 & 21 & 182.910 & 5.746 & 2.170 & -0.010 & 0.029 & 7.495 & 0.088 & 18.724 & 0.017 & 2.592 & 0.015 & 4.231 & 234.390 & 8.239 \\
Br22$^{\mathrm{SG}}$ & 89.615 & 7.758 & 18 & 18 & 33.245 & 94.476 & 1.399 & -0.215 & 0.103 & 7.200 & 0.014 & 0.563 & 0.012 & -0.389 & 0.010 & 0.134 & 5334.363 & 8.897 \\
Br30$^{\mathrm{SG}}$ & 104.436 & 3.227 & 11 & 11 & 28.260 & 46.485 & 2.028 & -0.140 & 0.148 & 7.390 & 0.014 & -0.218 & 0.007 & -0.313 & 0.006 & 0.176 & 4462.350 & 8.663 \\
Br31$^{\mathrm{SG}}$ & 104.406 & 8.288 & 49 & 49 & 31.030 & 56.582 & 1.981 & -0.370 & 0.103 & 7.260 & 0.014 & 0.114 & 0.008 & -0.921 & 0.006 & 0.122 & 5864.814 & 9.075 \\
Br36$^{\mathrm{SG}}$ & 109.100 & -13.193 & 104 & 104 & 27.365 & 62.833 & 1.756 & -0.190 & 0.148 & 7.359 & 0.185 & -1.692 & 0.006 & 0.957 & 0.004 & 0.212 & 3839.619 & 9.018 \\
Br44$^{\mathrm{SG}}$ & 289.314 & 19.548 & 37 & 37 & 50.160 & -8.481 & 1.529 & 0.120 & 0.103 & 7.785 & 0.059 & -0.052 & 0.005 & -2.878 & 0.006 & 0.343 & 2690.292 & 9.003 \\
Br75$^{\mathrm{SG}}$ & 102.248 & -23.995 & 21 & 21 & 26.470 & 124.357 & 2.184 & -0.600 & 0.163 & 7.220 & 0.074 & -0.241 & 0.006 & 1.178 & 0.010 & 0.107 & 6829.598 & 9.269 \\
Cz24$^{\mathrm{SG}}$ & 88.852 & 20.877 & 55 & 55 & 41.140 & 22.953 & 2.986 & -0.190 & 0.148 & 7.430 & 0.029 & 0.259 & 0.010 & -2.720 & 0.009 & 0.227 & 3722.727 & 9.080 \\
Cz30$^{\mathrm{SG}}$ & 112.795 & -9.946 & 46 & 46 & 32.635 & 81.935 & 1.516 & -0.425 & 0.177 & 7.260 & 0.059 & -0.612 & 0.008 & -0.065 & 0.008 & 0.133 & 6108.557 & 9.033 \\
M67$^{\mathrm{SG}}$ & 132.849 & 11.817 & 106 & 106 & 152.980 & 33.721 & 2.342 & -0.010 & 0.059 & 7.500 & 0.059 & -10.965 & 0.006 & -2.905 & 0.006 & 1.150 & 837.267 & 9.227 \\
NGC2232$^{\mathrm{SG}}$ & 96.977 & -4.771 & 7 & 7 & 134.160 & 26.714 & 2.164 & 0.020 & 0.029 & 7.540 & 0.000 & -4.716 & 0.015 & -1.769 & 0.016 & 3.119 & 318.036 & 7.123 \\
NGC2451$^{\mathrm{SG}}$ & 116.176 & -37.942 & 6 & 6 & 167.985 & 23.271 & 0.935 & -0.080 & 0.051 & 7.440 & 0.044 & -9.400 & 0.025 & 4.744 & 0.012 & 2.675 & 367.535 & 7.440 \\
NGC6005$^{\mathrm{SG}}$ & 238.950 & -57.435 & 31 & 31 & 46.320 & -24.932 & 1.404 & 0.170 & 0.088 & 7.710 & 0.029 & -4.035 & 0.004 & -3.813 & 0.004 & 0.386 & 2388.113 & 8.933 \\
NGC6067$^{\mathrm{SG}}$ & 243.295 & -54.231 & 58 & 58 & 89.580 & -38.171 & 2.088 & 0.070 & 0.103 & 7.720 & 0.088 & -1.960 & 0.003 & -2.578 & 0.003 & 0.471 & 1957.161 & 7.949 \\
NGC6259$^{\mathrm{SG}}$ & 255.192 & -44.676 & 32 & 32 & 66.785 & -32.438 & 2.490 & 0.165 & 0.103 & 7.845 & 0.081 & -1.046 & 0.003 & -2.892 & 0.003 & 0.424 & 2158.990 & 8.215 \\
NGC6281$^{\mathrm{SG}}$ & 256.188 & -37.940 & 32 & 32 & 77.555 & -4.465 & 0.794 & 0.030 & 0.103 & 7.475 & 0.037 & -1.880 & 0.010 & -4.049 & 0.010 & 1.885 & 520.762 & 8.437 \\
NGC6405$^{\mathrm{SG}}$ & 265.067 & -32.228 & 43 & 43 & 67.490 & -8.717 & 0.893 & 0.010 & 0.074 & 7.540 & 0.103 & -1.368 & 0.011 & -5.847 & 0.010 & 2.176 & 451.869 & 7.719 \\
NGC6633$^{\mathrm{SG}}$ & 276.805 & 6.559 & 21 & 21 & 102.270 & -28.602 & 2.061 & -0.060 & 0.103 & 7.590 & 0.103 & 1.204 & 0.016 & -1.803 & 0.016 & 2.540 & 389.528 & 8.674 \\
NGC6709$^{\mathrm{SG}}$ & 282.833 & 10.322 & 45 & 45 & 61.980 & -9.588 & 1.491 & -0.110 & 0.088 & 7.440 & 0.059 & 1.445 & 0.007 & -3.539 & 0.008 & 0.923 & 1048.055 & 8.207 \\
Pismis15$^{\mathrm{SG}}$ & 143.687 & -48.040 & 26 & 26 & 38.305 & 35.081 & 1.243 & -0.055 & 0.126 & 7.500 & 0.051 & -5.259 & 0.006 & 3.385 & 0.006 & 0.409 & 2254.343 & 8.652 \\
Pismis18$^{\mathrm{SG}}$ & 204.226 & -62.091 & 11 & 11 & 102.470 & -28.499 & 2.611 & 0.120 & 0.059 & 7.630 & 0.029 & -5.691 & 0.004 & -2.269 & 0.004 & 0.347 & 2598.111 & 8.508 \\
Trumpler23$^{\mathrm{SG}}$ & 240.213 & -53.537 & 20 & 20 & 74.565 & -61.407 & 2.189 & 0.175 & 0.066 & 7.814 & 0.037 & -4.210 & 0.004 & -4.758 & 0.004 & 0.366 & 2471.292 & 8.520 \\
gamma2\_Vel$^{\mathrm{SG}}$ & 122.374 & -47.353 & 4 & 4 & 213.825 & 19.467 & 2.207 & 0.050 & 0.037 & 7.490 & 0.000 & -6.363 & 0.016 & 9.436 & 0.028 & 2.846 & 346.884 & 6.971 \\
Br21$^{\mathrm{S}}$ & 87.948 & 21.810 & 60 & 60 & 31.400 & 1.494 & 4.609 & -0.195 & 0.163 & 7.340 & 0.155 & 0.506 & 0.009 & -1.031 & 0.008 & 0.143 & 5294.645 & 8.945 \\
Br32$^{\mathrm{S}}$ & 104.531 & 6.433 & 169 & 169 & 41.120 & 106.146 & 3.164 & -0.390 & 0.118 & 7.261 & 0.059 & -0.356 & 0.005 & -1.589 & 0.004 & 0.274 & 3147.859 & 9.512 \\
Br39$^{\mathrm{S}}$ & 116.707 & -4.672 & 330 & 330 & 38.114 & 58.979 & 3.211 & -0.240 & 0.133 & 7.450 & 0.029 & -1.731 & 0.003 & -1.631 & 0.003 & 0.230 & 3809.337 & 9.494 \\
Br73$^{\mathrm{S}}$ & 95.520 & -6.318 & 15 & 15 & 37.840 & 97.290 & 3.650 & -0.240 & 0.103 & 7.290 & 0.029 & 0.213 & 0.010 & 1.012 & 0.015 & 0.121 & 6497.806 & 9.128 \\
Br81$^{\mathrm{S}}$ & 285.416 & -0.457 & 19 & 19 & 37.150 & 48.322 & 3.341 & 0.120 & 0.103 & 7.685 & 0.066 & -1.144 & 0.008 & -1.961 & 0.009 & 0.251 & 3468.979 & 8.352 \\
Col197$^{\mathrm{S}}$ & 131.215 & -41.260 & 3 & 3 & 61.320 & 20.703 & 3.467 & 0.100 & 0.074 & 7.540 & 0.000 & -5.735 & 0.014 & 4.075 & 0.012 & 1.038 & 924.127 & 6.605 \\
ESO92\_05$^{\mathrm{S}}$ & 150.789 & -64.754 & 12 & 12 & 27.520 & 59.686 & 4.148 & -0.425 & 0.066 & $\cdots$ & $\cdots$ & -3.023 & 0.018 & 2.461 & 0.011 & 0.058 & 11149.450 & 9.199 \\
IC4665$^{\mathrm{S}}$ & 266.532 & 5.634 & 13 & 13 & 113.700 & -13.230 & 6.252 & 0.000 & 0.059 & 7.560 & 0.266 & -0.880 & 0.018 & -8.532 & 0.018 & 2.866 & 343.345 & 7.514 \\
NGC2141$^{\mathrm{S}}$ & 90.744 & 10.455 & 380 & 380 & 37.550 & 26.834 & 4.950 & -0.100 & 0.088 & 7.470 & 0.044 & -0.082 & 0.003 & -0.754 & 0.002 & 0.203 & 4052.221 & 9.262 \\
NGC2158$^{\mathrm{S}}$ & 91.859 & 24.097 & 210 & 210 & 41.425 & 28.521 & 3.854 & -0.210 & 0.133 & 7.400 & 0.059 & -0.210 & 0.003 & -1.982 & 0.002 & 0.232 & 3706.334 & 9.269 \\
NGC2243$^{\mathrm{S}}$ & 97.396 & -31.283 & 332 & 332 & 36.269 & 59.522 & 3.081 & -0.625 & 0.148 & 7.068 & 0.091 & -1.267 & 0.003 & 5.493 & 0.003 & 0.222 & 3928.227 & 9.439 \\
NGC2244$^{\mathrm{S}}$ & 97.985 & 4.926 & 2 & 2 & 36.035 & 28.155 & 5.084 & -0.035 & 0.007 & $\cdots$ & $\cdots$ & -1.736 & 0.008 & 0.252 & 0.009 & 0.656 & 1415.235 & 6.613 \\
NGC2264$^{\mathrm{S}}$ & 100.273 & 9.572 & 8 & 8 & 119.350 & 20.068 & 4.939 & -0.065 & 0.044 & 7.564 & 0.155 & -2.377 & 0.017 & -3.722 & 0.015 & 1.377 & 706.459 & 6.756 \\
NGC2355$^{\mathrm{S}}$ & 109.250 & 13.762 & 79 & 79 & 52.060 & 36.383 & 5.770 & -0.120 & 0.059 & 7.340 & 0.029 & -3.836 & 0.005 & -1.054 & 0.004 & 0.525 & 1751.095 & 9.232 \\
NGC2420$^{\mathrm{S}}$ & 114.602 & 21.574 & 311 & 311 & 60.530 & 74.065 & 5.446 & -0.220 & 0.088 & 7.279 & 0.084 & -1.214 & 0.003 & -2.039 & 0.003 & 0.390 & 2311.418 & 9.352 \\
NGC2425$^{\mathrm{S}}$ & 114.579 & -14.888 & 114 & 114 & 51.885 & 103.764 & 3.271 & -0.205 & 0.111 & 7.380 & 0.081 & -3.573 & 0.004 & 2.011 & 0.004 & 0.283 & 3094.027 & 9.295 \\
NGC2516$^{\mathrm{S}}$ & 119.521 & -60.792 & 310 & 310 & 63.690 & 23.994 & 3.709 & 0.000 & 0.074 & 7.610 & 0.252 & -4.633 & 0.010 & 11.225 & 0.008 & 2.427 & 407.088 & 8.097 \\
NGC2547$^{\mathrm{S}}$ & 122.533 & -49.194 & 25 & 25 & 154.460 & 13.268 & 3.575 & 0.000 & 0.059 & 7.689 & 0.155 & -8.567 & 0.012 & 4.330 & 0.012 & 2.574 & 382.382 & 7.336 \\
NGC3532$^{\mathrm{S}}$ & 166.393 & -58.693 & 368 & 368 & 107.530 & 5.412 & 4.522 & 0.010 & 0.074 & 7.401 & 0.120 & -10.402 & 0.007 & 5.228 & 0.007 & 2.087 & 471.884 & 8.376 \\
NGC4815$^{\mathrm{S}}$ & 194.507 & -64.959 & 29 & 29 & 32.150 & -28.007 & 5.716 & 0.050 & 0.103 & 7.560 & 0.007 & -5.809 & 0.003 & -0.934 & 0.003 & 0.286 & 3142.276 & 8.411 \\
NGC6253$^{\mathrm{S}}$ & 254.770 & -52.714 & 130 & 130 & 94.095 & -28.373 & 3.211 & 0.320 & 0.059 & 7.812 & 0.070 & -4.555 & 0.004 & -5.293 & 0.004 & 0.583 & 1606.201 & 9.267 \\
NGC6802$^{\mathrm{S}}$ & 292.646 & 20.258 & 40 & 40 & 42.770 & 14.643 & 4.162 & 0.060 & 0.118 & 7.615 & 0.044 & -2.846 & 0.004 & -6.454 & 0.004 & 0.326 & 2768.780 & 8.534 \\
Rup134$^{\mathrm{S}}$ & 268.175 & -29.534 & 80 & 80 & 71.085 & -40.707 & 5.072 & 0.175 & 0.118 & 7.830 & 0.059 & -1.606 & 0.007 & -2.440 & 0.007 & 0.391 & 2296.640 & 8.308 \\
Trumpler14$^{\mathrm{S}}$ & 161.264 & -59.696 & 27 & 27 & 45.700 & -10.043 & 8.061 & -0.040 & 0.074 & $\cdots$ & $\cdots$ & -6.908 & 0.010 & 2.606 & 0.009 & 0.402 & 2296.983 & 6.794 \\
Trumpler20$^{\mathrm{S}}$ & 189.887 & -60.632 & 187 & 187 & 44.740 & -40.228 & 3.415 & 0.080 & 0.088 & 7.590 & 0.044 & -7.109 & 0.002 & 0.193 & 0.002 & 0.271 & 3279.385 & 9.200 \\
Trumpler5$^{\mathrm{S}}$ & 99.127 & 9.458 & 524 & 524 & 35.265 & 51.422 & 5.010 & -0.470 & 0.148 & 7.230 & 0.029 & -0.617 & 0.002 & 0.269 & 0.002 & 0.302 & 2904.927 & 9.337 \\
lam\_Ori$^{\mathrm{S}}$ & 83.814 & 9.888 & 5 & 5 & 123.420 & 26.574 & 3.055 & -0.010 & 0.133 & 7.410 & 0.148 & 1.214 & 0.019 & -2.046 & 0.016 & 2.503 & 393.775 & 6.719 \\
25\_Ori & 81.083 & 1.695 & 6 & 6 & 243.305 & 15.621 & 8.766 & 0.020 & 0.051 & 7.470 & 0.000 & 1.383 & 0.013 & -0.016 & 0.013 & 2.887 & 342.098 & 6.913 \\
Assc50 & 132.576 & -41.691 & 4 & 4 & 70.075 & 29.460 & 14.221 & -0.105 & 0.103 & 7.300 & 0.000 & -5.549 & 0.012 & 3.953 & 0.014 & 1.060 & 917.830 & 6.641 \\
Cha\_I & 167.116 & -77.499 & 1 & 1 & 242.120 & 14.400 & $\cdots$ & 0.240 & 0.000 & 7.540 & 0.000 & -22.555 & 0.055 & 0.437 & 0.078 & 5.261 & 188.665 & 6.753 \\
Haf10 & 112.148 & -15.364 & 166 & 166 & 34.690 & 86.393 & 9.240 & -0.240 & 0.163 & 7.415 & 0.044 & -1.203 & 0.004 & 1.559 & 0.005 & 0.264 & 3453.648 & 8.514 \\
IC2391 & 130.260 & -53.041 & 7 & 7 & 226.540 & 19.805 & 6.112 & -0.100 & 0.311 & 7.330 & 0.014 & -24.796 & 0.055 & 23.267 & 0.046 & 6.621 & 150.190 & 7.436 \\
IC2602 & 160.973 & -64.393 & 12 & 12 & 250.945 & 23.130 & 10.824 & -0.035 & 0.111 & 7.620 & 0.088 & -17.775 & 0.055 & 10.669 & 0.053 & 6.600 & 150.551 & 7.414 \\
NGC6530 & 271.101 & -24.370 & 4 & 4 & 82.130 & -5.720 & 19.635 & -0.110 & 0.185 & $\cdots$ & $\cdots$ & 1.333 & 0.015 & -2.058 & 0.010 & 0.764 & 1229.501 & 6.591 \\
NGC6649 & 278.358 & -10.402 & 3 & 3 & 54.680 & -6.803 & 11.248 & -0.150 & 0.059 & $\cdots$ & $\cdots$ & 0.037 & 0.004 & -0.114 & 0.005 & 0.473 & 1960.505 & 7.448 \\
NGC6705 & 282.765 & -6.275 & 228 & 228 & 46.995 & 35.656 & 9.049 & 0.040 & 0.103 & 7.715 & 0.096 & -1.535 & 0.003 & -4.165 & 0.003 & 0.411 & 2233.066 & 8.119 \\
\end{longtable}


==> table_orbital_parameters_science.tex <==
\begin{longtable}{lcccccccccccccccccccccc}
\caption{Derived orbital parameters for the SCIENCE sample of Gaia--ESO open clusters. Columns give heliocentric distance ($d$; pc), age (Gyr), pericentre and apocentre radii (kpc), orbital eccentricity, maximum vertical excursion (kpc), orbital actions ($J_R$, $J_{\phi}$, $J_Z$; kpc\,km\,s$^{-1}$), and guiding radius (kpc). Uncertainties are 1$\sigma$.} \label{tab:orbital_parameters_science} \\
\toprule
GES\_FLD &
$d$ &
$\sigma_d$ &
$\log\,\mathrm{Age}$ &
$\sigma_{\log\mathrm{Age}}$ &
$\mathrm{Age}$ &
$\sigma_{\mathrm{Age}}$ &
$R_{\mathrm{peri}}$ &
$\sigma_{R_{\mathrm{peri}}}$ &
$R_{\mathrm{apo}}$ &
$\sigma_{R_{\mathrm{apo}}}$ &
$e$ &
$\sigma_e$ &
$Z_{\max}$ &
$\sigma_{Z_{\max}}$ &
$J_R$ &
$\sigma_{J_R}$ &
$J_{\phi}$ &
$\sigma_{J_{\phi}}$ &
$J_Z$ &
$\sigma_{J_Z}$ &
$R_g$ &
$\sigma_{R_g}$ \\
\midrule
 &
(pc) &
(pc) &
(-) &
(-) &
(Gyr) &
(Gyr) &
(kpc) &
(kpc) &
(kpc) &
(kpc) &
(–) &
(–) &
(kpc) &
(kpc) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc) &
(kpc) \\
\midrule
\endfirsthead
\caption[]{Derived orbital parameters for the SCIENCE sample of Gaia--ESO open clusters. Columns give heliocentric distance ($d$; pc), age (Gyr), pericentre and apocentre radii (kpc), orbital eccentricity, maximum vertical excursion (kpc), orbital actions ($J_R$, $J_{\phi}$, $J_Z$; kpc\,km\,s$^{-1}$), and guiding radius (kpc). Uncertainties are 1$\sigma$. Values are truncated to three decimal places.} \\
\toprule
GES\_FLD &
$d$ &
$\sigma_d$ &
$\log\,\mathrm{Age}$ &
$\sigma_{\log\mathrm{Age}}$ &
$\mathrm{Age}$ &
$\sigma_{\mathrm{Age}}$ &
$R_{\mathrm{peri}}$ &
$\sigma_{R_{\mathrm{peri}}}$ &
$R_{\mathrm{apo}}$ &
$\sigma_{R_{\mathrm{apo}}}$ &
$e$ &
$\sigma_e$ &
$Z_{\max}$ &
$\sigma_{Z_{\max}}$ &
$J_R$ &
$\sigma_{J_R}$ &
$J_{\phi}$ &
$\sigma_{J_{\phi}}$ &
$J_Z$ &
$\sigma_{J_Z}$ &
$R_g$ &
$\sigma_{R_g}$ \\

\midrule
\endhead
\midrule
\multicolumn{23}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Blanco1 & 234.390 & 0.094 & 8.239 & 0.309 & 0.173 & 0.140 & 8.079 & 0.004 & 8.713 & 0.001 & 0.037 & 0.000 & 0.215 & 0.001 & 1.867 & 0.021 & 1938.128 & 0.520 & 1.551 & 0.019 & 8.371 & 0.002 \\
Br21 & 5294.645 & 152.808 & 8.945 & 0.255 & 0.881 & 0.606 & 12.240 & 0.135 & 14.211 & 0.215 & 0.074 & 0.010 & 0.235 & 0.007 & 10.722 & 2.986 & 2888.963 & 21.462 & 0.949 & 0.041 & 13.157 & 0.111 \\
Br22 & 5334.363 & 128.064 & 8.897 & 0.263 & 0.789 & 0.545 & 10.910 & 0.257 & 14.559 & 0.221 & 0.143 & 0.017 & 0.789 & 0.020 & 38.060 & 9.047 & 2749.343 & 25.489 & 7.940 & 0.281 & 12.436 & 0.131 \\
Br30 & 4462.350 & 73.578 & 8.663 & 0.180 & 0.460 & 0.190 & 11.439 & 0.114 & 12.697 & 0.469 & 0.050 & 0.019 & 0.278 & 0.007 & 4.426 & 4.838 & 2672.182 & 40.891 & 1.518 & 0.030 & 12.039 & 0.209 \\
Br31 & 5864.814 & 174.234 & 9.075 & 0.228 & 1.190 & 0.708 & 10.954 & 0.180 & 13.708 & 0.174 & 0.111 & 0.007 & 0.587 & 0.015 & 22.195 & 3.176 & 2693.462 & 29.961 & 5.216 & 0.146 & 12.148 & 0.153 \\
Br32 & 3147.859 & 21.970 & 9.512 & 0.150 & 3.252 & 1.213 & 7.219 & 0.086 & 11.831 & 0.057 & 0.242 & 0.007 & 0.289 & 0.002 & 85.394 & 5.436 & 2069.601 & 9.988 & 1.771 & 0.020 & 9.010 & 0.048 \\
Br36 & 3839.619 & 48.311 & 9.018 & 0.182 & 1.042 & 0.443 & 11.048 & 0.050 & 11.370 & 0.139 & 0.014 & 0.005 & 0.258 & 0.008 & 0.343 & 0.295 & 2506.479 & 16.260 & 1.545 & 0.077 & 11.193 & 0.082 \\
Br39 & 3809.337 & 30.210 & 9.494 & 0.149 & 3.125 & 1.133 & 8.245 & 0.027 & 11.363 & 0.031 & 0.158 & 0.001 & 0.999 & 0.016 & 37.032 & 0.484 & 2158.078 & 5.148 & 16.377 & 0.339 & 9.445 & 0.025 \\
Br44 & 2690.292 & 20.772 & 9.003 & 0.182 & 1.008 & 0.470 & 5.511 & 0.122 & 7.376 & 0.019 & 0.144 & 0.009 & 0.223 & 0.002 & 21.829 & 2.695 & 1493.761 & 19.283 & 2.038 & 0.044 & 6.306 & 0.085 \\
Br73 & 6497.806 & 279.208 & 9.128 & 0.176 & 1.343 & 0.562 & 13.314 & 0.380 & 15.805 & 0.440 & 0.086 & 0.006 & 1.304 & 0.085 & 15.779 & 2.348 & 3111.288 & 74.399 & 17.148 & 1.319 & 14.315 & 0.389 \\
Br75 & 6829.598 & 290.963 & 9.269 & 0.205 & 1.858 & 0.996 & 9.710 & 0.391 & 13.464 & 0.237 & 0.162 & 0.011 & 1.326 & 0.051 & 44.743 & 5.267 & 2496.357 & 65.916 & 21.093 & 0.989 & 11.141 & 0.334 \\
Br81 & 3468.979 & 46.229 & 8.352 & 0.207 & 0.225 & 0.112 & 5.535 & 0.063 & 6.293 & 0.087 & 0.064 & 0.003 & 0.159 & 0.002 & 4.108 & 0.453 & 1397.674 & 16.580 & 1.289 & 0.043 & 5.883 & 0.072 \\
Col197 & 924.127 & 1.751 & 6.605 & 0.109 & 0.004 & 0.000 & 8.204 & 0.251 & 8.447 & 0.207 & 0.021 & 0.013 & 0.043 & 0.001 & 0.584 & 1.206 & 1928.107 & 43.010 & 0.068 & 0.001 & 8.323 & 0.206 \\
Cz24 & 3722.727 & 90.968 & 9.080 & 0.180 & 1.203 & 0.502 & 9.280 & 0.027 & 11.969 & 0.117 & 0.126 & 0.005 & 0.346 & 0.019 & 25.298 & 2.297 & 2360.600 & 8.570 & 2.440 & 0.224 & 10.455 & 0.043 \\
Cz30 & 6108.557 & 169.368 & 9.033 & 0.189 & 1.081 & 0.487 & 10.157 & 0.145 & 13.328 & 0.173 & 0.135 & 0.001 & 0.493 & 0.015 & 31.485 & 0.724 & 2570.502 & 30.757 & 3.940 & 0.153 & 11.519 & 0.156 \\
ESO92\_05 & 11149.450 & 574.221 & 9.199 & 0.338 & 1.584 & 1.412 & 9.984 & 0.676 & 16.133 & 3.108 & 0.237 & 0.065 & 1.932 & 0.302 & 105.846 & 99.093 & 2693.215 & 242.282 & 30.886 & 2.077 & 12.147 & 1.243 \\
IC4665 & 343.345 & 0.239 & 7.514 & 0.230 & 0.032 & 0.017 & 7.383 & 0.089 & 7.922 & 0.007 & 0.035 & 0.006 & 0.129 & 0.002 & 1.464 & 0.529 & 1784.086 & 10.425 & 0.654 & 0.026 & 7.637 & 0.049 \\
M67 & 837.267 & 0.628 & 9.227 & 0.178 & 1.688 & 0.737 & 7.789 & 0.010 & 9.295 & 0.002 & 0.088 & 0.000 & 0.560 & 0.001 & 10.115 & 0.181 & 1946.596 & 1.085 & 8.009 & 0.037 & 8.412 & 0.005 \\
NGC2141 & 4052.221 & 34.795 & 9.262 & 0.154 & 1.831 & 0.707 & 11.710 & 0.046 & 12.967 & 0.096 & 0.050 & 0.005 & 0.410 & 0.004 & 4.671 & 0.963 & 2720.446 & 7.263 & 3.003 & 0.046 & 12.287 & 0.037 \\
NGC2158 & 3706.334 & 20.611 & 9.269 & 0.160 & 1.858 & 0.704 & 10.799 & 0.026 & 11.932 & 0.025 & 0.049 & 0.001 & 0.325 & 0.004 & 4.111 & 0.316 & 2531.236 & 2.864 & 2.213 & 0.046 & 11.319 & 0.014 \\
NGC2232 & 318.036 & 0.224 & 7.123 & 0.234 & 0.013 & 0.007 & 8.437 & 0.029 & 8.616 & 0.031 & 0.011 & 0.001 & 0.045 & 0.002 & 0.160 & 0.043 & 1969.963 & 5.964 & 0.073 & 0.006 & 8.525 & 0.028 \\
NGC2243 & 3928.227 & 23.567 & 9.439 & 0.167 & 2.748 & 1.115 & 10.445 & 0.019 & 16.863 & 0.124 & 0.234 & 0.002 & 1.838 & 0.022 & 109.860 & 2.952 & 2815.872 & 10.129 & 26.733 & 0.271 & 12.779 & 0.052 \\
NGC2244 & 1415.235 & 4.221 & 6.613 & 0.122 & 0.004 & 0.001 & 9.451 & 0.129 & 10.393 & 0.238 & 0.050 & 0.010 & 0.060 & 0.003 & 3.727 & 2.122 & 2251.631 & 30.092 & 0.103 & 0.014 & 9.910 & 0.150 \\
NGC2264 & 706.459 & 1.968 & 6.756 & 0.157 & 0.005 & 0.002 & 8.652 & 0.186 & 8.950 & 0.199 & 0.020 & 0.016 & 0.085 & 0.004 & 0.590 & 1.664 & 2023.196 & 26.543 & 0.253 & 0.019 & 8.783 & 0.129 \\
NGC2355 & 1751.095 & 5.018 & 9.232 & 0.171 & 1.706 & 0.674 & 9.754 & 0.110 & 10.906 & 0.176 & 0.057 & 0.007 & 0.599 & 0.033 & 5.286 & 1.676 & 2316.546 & 22.900 & 7.534 & 0.504 & 10.234 & 0.114 \\
NGC2420 & 2311.418 & 8.766 & 9.352 & 0.169 & 2.250 & 0.908 & 8.222 & 0.074 & 11.303 & 0.062 & 0.157 & 0.007 & 0.918 & 0.010 & 36.508 & 3.306 & 2153.989 & 5.499 & 14.210 & 0.151 & 9.425 & 0.027 \\
NGC2425 & 3094.027 & 21.859 & 9.295 & 0.160 & 1.975 & 0.729 & 8.202 & 0.050 & 11.593 & 0.032 & 0.171 & 0.002 & 0.490 & 0.008 & 43.723 & 1.177 & 2188.967 & 8.245 & 4.731 & 0.118 & 9.598 & 0.040 \\
NGC2451 & 367.535 & 0.148 & 7.440 & 0.223 & 0.027 & 0.015 & 8.305 & 0.001 & 8.857 & 0.094 & 0.032 & 0.005 & 0.063 & 0.001 & 1.369 & 0.464 & 1979.672 & 9.097 & 0.140 & 0.008 & 8.572 & 0.044 \\
NGC2516 & 407.088 & 0.089 & 8.097 & 0.269 & 0.125 & 0.089 & 7.310 & 0.021 & 8.183 & 0.000 & 0.056 & 0.001 & 0.095 & 0.000 & 3.861 & 0.198 & 1801.942 & 2.523 & 0.344 & 0.003 & 7.721 & 0.011 \\
NGC2547 & 382.382 & 0.179 & 7.336 & 0.259 & 0.021 & 0.014 & 8.190 & 0.011 & 8.764 & 0.127 & 0.033 & 0.006 & 0.053 & 0.002 & 1.501 & 0.626 & 1958.170 & 13.602 & 0.100 & 0.010 & 8.468 & 0.065 \\
NGC3532 & 471.884 & 0.109 & 8.376 & 0.249 & 0.237 & 0.155 & 7.988 & 0.020 & 8.062 & 0.001 & 0.004 & 0.001 & 0.121 & 0.000 & 0.025 & 0.014 & 1864.877 & 2.262 & 0.566 & 0.002 & 8.020 & 0.010 \\
NGC4815 & 3142.276 & 12.634 & 8.411 & 0.174 & 0.258 & 0.109 & 6.558 & 0.112 & 7.118 & 0.033 & 0.040 & 0.006 & 0.103 & 0.000 & 1.840 & 0.609 & 1608.696 & 16.518 & 0.480 & 0.007 & 6.824 & 0.075 \\
NGC6005 & 2388.113 & 9.511 & 8.933 & 0.171 & 0.857 & 0.339 & 4.935 & 0.070 & 6.374 & 0.007 & 0.127 & 0.007 & 0.115 & 0.000 & 15.206 & 1.619 & 1324.177 & 10.244 & 0.671 & 0.008 & 5.567 & 0.043 \\
NGC6067 & 1957.161 & 3.378 & 7.949 & 0.187 & 0.088 & 0.040 & 6.580 & 0.011 & 6.901 & 0.106 & 0.023 & 0.007 & 0.070 & 0.001 & 0.608 & 0.469 & 1589.522 & 10.960 & 0.236 & 0.005 & 6.737 & 0.049 \\
NGC6253 & 1606.201 & 3.190 & 9.267 & 0.167 & 1.852 & 0.779 & 5.335 & 0.016 & 6.849 & 0.007 & 0.124 & 0.000 & 0.216 & 0.001 & 15.333 & 0.222 & 1422.510 & 2.967 & 2.091 & 0.018 & 5.992 & 0.012 \\
NGC6259 & 2158.990 & 3.723 & 8.215 & 0.178 & 0.164 & 0.070 & 5.721 & 0.020 & 6.227 & 0.020 & 0.042 & 0.000 & 0.041 & 0.000 & 1.780 & 0.051 & 1416.017 & 4.592 & 0.090 & 0.001 & 5.963 & 0.020 \\
NGC6281 & 520.762 & 0.338 & 8.437 & 0.234 & 0.273 & 0.161 & 7.574 & 0.013 & 7.921 & 0.006 & 0.022 & 0.001 & 0.072 & 0.000 & 0.605 & 0.068 & 1806.311 & 0.859 & 0.207 & 0.001 & 7.742 & 0.004 \\
NGC6405 & 451.869 & 0.274 & 7.719 & 0.240 & 0.052 & 0.030 & 7.700 & 0.018 & 7.759 & 0.015 & 0.003 & 0.002 & 0.043 & 0.000 & 0.017 & 0.033 & 1803.377 & 0.657 & 0.077 & 0.001 & 7.728 & 0.003 \\
NGC6633 & 389.528 & 0.201 & 8.674 & 0.212 & 0.472 & 0.248 & 7.212 & 0.034 & 8.133 & 0.004 & 0.060 & 0.002 & 0.082 & 0.000 & 4.348 & 0.379 & 1785.875 & 3.570 & 0.260 & 0.000 & 7.646 & 0.016 \\
NGC6709 & 1048.055 & 1.571 & 8.207 & 0.210 & 0.161 & 0.088 & 7.030 & 0.155 & 7.561 & 0.009 & 0.036 & 0.011 & 0.146 & 0.002 & 1.515 & 1.030 & 1707.541 & 17.164 & 0.882 & 0.027 & 7.279 & 0.079 \\
NGC6802 & 2768.780 & 13.561 & 8.534 & 0.175 & 0.342 & 0.145 & 6.305 & 0.132 & 7.450 & 0.133 & 0.084 & 0.003 & 0.067 & 0.000 & 7.856 & 0.639 & 1610.858 & 29.043 & 0.193 & 0.001 & 6.834 & 0.132 \\
Pismis15 & 2254.343 & 10.105 & 8.652 & 0.182 & 0.448 & 0.201 & 7.215 & 0.159 & 8.421 & 0.005 & 0.077 & 0.010 & 0.140 & 0.000 & 7.289 & 1.983 & 1812.396 & 19.757 & 0.708 & 0.007 & 7.771 & 0.093 \\
Pismis18 & 2598.111 & 12.083 & 8.508 & 0.184 & 0.322 & 0.154 & 6.502 & 0.036 & 6.919 & 0.004 & 0.031 & 0.002 & 0.090 & 0.000 & 1.037 & 0.181 & 1581.745 & 4.387 & 0.385 & 0.007 & 6.701 & 0.019 \\
Rup134 & 2296.640 & 12.284 & 8.308 & 0.218 & 0.203 & 0.104 & 4.534 & 0.093 & 6.241 & 0.160 & 0.158 & 0.022 & 0.109 & 0.005 & 22.591 & 6.904 & 1252.751 & 3.717 & 0.631 & 0.038 & 5.265 & 0.015 \\
Trumpler14 & 2296.983 & 6.845 & 6.794 & 0.208 & 0.006 & 0.003 & 7.789 & 0.509 & 7.832 & 0.630 & 0.043 & 0.036 & 0.030 & 0.001 & 2.325 & 6.472 & 1820.377 & 102.753 & 0.037 & 0.005 & 7.809 & 0.486 \\
Trumpler20 & 3279.385 & 10.675 & 9.200 & 0.163 & 1.584 & 0.592 & 7.014 & 0.002 & 7.750 & 0.028 & 0.049 & 0.001 & 0.162 & 0.000 & 2.923 & 0.209 & 1724.141 & 3.025 & 1.040 & 0.005 & 7.356 & 0.014 \\
Trumpler23 & 2471.292 & 10.055 & 8.520 & 0.164 & 0.331 & 0.123 & 5.042 & 0.091 & 6.399 & 0.065 & 0.118 & 0.004 & 0.018 & 0.000 & 13.424 & 0.842 & 1343.303 & 19.057 & 0.017 & 0.001 & 5.649 & 0.081 \\
Trumpler5 & 2904.927 & 9.492 & 9.337 & 0.166 & 2.173 & 0.850 & 10.702 & 0.019 & 12.289 & 0.014 & 0.069 & 0.000 & 0.104 & 0.000 & 8.113 & 0.182 & 2556.112 & 2.946 & 0.242 & 0.001 & 11.445 & 0.015 \\
gamma2\_Vel & 346.884 & 0.166 & 6.971 & 0.225 & 0.009 & 0.004 & 8.248 & 0.074 & 8.338 & 0.140 & 0.008 & 0.007 & 0.067 & 0.004 & 0.088 & 0.307 & 1921.525 & 18.842 & 0.169 & 0.019 & 8.291 & 0.090 \\
lam\_Ori & 393.775 & 0.213 & 6.719 & 0.157 & 0.005 & 0.001 & 8.527 & 0.037 & 8.948 & 0.011 & 0.023 & 0.002 & 0.071 & 0.003 & 0.774 & 0.155 & 2012.117 & 4.313 & 0.175 & 0.017 & 8.729 & 0.020 \\
\end{longtable}

==> table_orbital_parameters_science_unchanged.tex <==

\begin{longtable}{lcccccccccccccccccccccccc}
\caption{Derived orbital parameters for the SCIENCE sample of Gaia--ESO open clusters. Columns give heliocentric distance ($d$; pc), sky position (ICRS), age (Gyr), pericentre and apocentre radii (kpc), orbital eccentricity, maximum vertical excursion (kpc), orbital actions ($J_R$, $J_{\phi}$, $J_Z$; kpc\,km\,s$^{-1}$), and guiding radius (kpc). Uncertainties are 1$\sigma$.} \label{tab:orbital_parameters_science} \\
\toprule
GES\_FLD &
$\mathrm{RA}$ &
$\mathrm{Dec}$ &
$d$ &
$\sigma_d$ &
$\log\,\mathrm{Age}$ &
$\sigma_{\log\mathrm{Age}}$ &
$\mathrm{Age}$ &
$\sigma_{\mathrm{Age}}$ &
$R_{\mathrm{peri}}$ &
$\sigma_{R_{\mathrm{peri}}}$ &
$R_{\mathrm{apo}}$ &
$\sigma_{R_{\mathrm{apo}}}$ &
$e$ &
$\sigma_e$ &
$Z_{\max}$ &
$\sigma_{Z_{\max}}$ &
$J_R$ &
$\sigma_{J_R}$ &
$J_{\phi}$ &
$\sigma_{J_{\phi}}$ &
$J_Z$ &
$\sigma_{J_Z}$ &
$R_g$ &
$\sigma_{R_g}$ \\
\midrule
 &
(deg) &
(deg) &
(pc) &
(pc) &
(-) &
(-) &
(Gyr) &
(Gyr) &
(kpc) &
(kpc) &
(kpc) &
(kpc) &
(–) &
(–) &
(kpc) &
(kpc) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc\,km\,s$^{-1}$) &
(kpc) &
(kpc) \\
\midrule
\endfirsthead
\caption[]{Derived orbital parameters for the SCIENCE sample of Gaia--ESO open clusters. Columns give heliocentric distance ($d$; pc), sky position (ICRS), age (Gyr), pericentre and apocentre radii (kpc), orbital eccentricity, maximum vertical excursion (kpc), orbital actions ($J_R$, $J_{\phi}$, $J_Z$; kpc\,km\,s$^{-1}$), and guiding radius (kpc). Uncertainties are 1$\sigma$. Values are truncated to three decimal places.} \\
\toprule
GES\_FLD &
$\mathrm{RA}$ &
$\mathrm{Dec}$ &
$d$ &
$\sigma_d$ &
$\log\,\mathrm{Age}$ &
$\sigma_{\log\mathrm{Age}}$ &
$\mathrm{Age}$ &
$\sigma_{\mathrm{Age}}$ &
$R_{\mathrm{peri}}$ &
$\sigma_{R_{\mathrm{peri}}}$ &
$R_{\mathrm{apo}}$ &
$\sigma_{R_{\mathrm{apo}}}$ &
$e$ &
$\sigma_e$ &
$Z_{\max}$ &
$\sigma_{Z_{\max}}$ &
$J_R$ &
$\sigma_{J_R}$ &
$J_{\phi}$ &
$\sigma_{J_{\phi}}$ &
$J_Z$ &
$\sigma_{J_Z}$ &
$R_g$ &
$\sigma_{R_g}$ \\

\midrule
\endhead
\midrule
\multicolumn{25}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
Blanco1 & 0.914 & -30.010 & 234.390 & 0.094 & 8.239 & 0.309 & 0.173 & 0.140 & 8.079 & 0.004 & 8.713 & 0.001 & 0.037 & 0.000 & 0.215 & 0.001 & 1.867 & 0.021 & 1938.128 & 0.520 & 1.551 & 0.019 & 8.371 & 0.002 \\
Br21 & 87.948 & 21.810 & 5294.645 & 152.808 & 8.945 & 0.255 & 0.881 & 0.606 & 12.240 & 0.135 & 14.211 & 0.215 & 0.074 & 0.010 & 0.235 & 0.007 & 10.722 & 2.986 & 2888.963 & 21.462 & 0.949 & 0.041 & 13.157 & 0.111 \\
Br22 & 89.615 & 7.758 & 5334.363 & 128.064 & 8.897 & 0.263 & 0.789 & 0.545 & 10.910 & 0.257 & 14.559 & 0.221 & 0.143 & 0.017 & 0.789 & 0.020 & 38.060 & 9.047 & 2749.343 & 25.489 & 7.940 & 0.281 & 12.436 & 0.131 \\
Br30 & 104.436 & 3.227 & 4462.350 & 73.578 & 8.663 & 0.180 & 0.460 & 0.190 & 11.439 & 0.114 & 12.697 & 0.469 & 0.050 & 0.019 & 0.278 & 0.007 & 4.426 & 4.838 & 2672.182 & 40.891 & 1.518 & 0.030 & 12.039 & 0.209 \\
Br31 & 104.406 & 8.288 & 5864.814 & 174.234 & 9.075 & 0.228 & 1.190 & 0.708 & 10.954 & 0.180 & 13.708 & 0.174 & 0.111 & 0.007 & 0.587 & 0.015 & 22.195 & 3.176 & 2693.462 & 29.961 & 5.216 & 0.146 & 12.148 & 0.153 \\
Br32 & 104.531 & 6.433 & 3147.859 & 21.970 & 9.512 & 0.150 & 3.252 & 1.213 & 7.219 & 0.086 & 11.831 & 0.057 & 0.242 & 0.007 & 0.289 & 0.002 & 85.394 & 5.436 & 2069.601 & 9.988 & 1.771 & 0.020 & 9.010 & 0.048 \\
Br36 & 109.100 & -13.193 & 3839.619 & 48.311 & 9.018 & 0.182 & 1.042 & 0.443 & 11.048 & 0.050 & 11.370 & 0.139 & 0.014 & 0.005 & 0.258 & 0.008 & 0.343 & 0.295 & 2506.479 & 16.260 & 1.545 & 0.077 & 11.193 & 0.082 \\
Br39 & 116.707 & -4.672 & 3809.337 & 30.210 & 9.494 & 0.149 & 3.125 & 1.133 & 8.245 & 0.027 & 11.363 & 0.031 & 0.158 & 0.001 & 0.999 & 0.016 & 37.032 & 0.484 & 2158.078 & 5.148 & 16.377 & 0.339 & 9.445 & 0.025 \\
Br44 & 289.314 & 19.548 & 2690.292 & 20.772 & 9.003 & 0.182 & 1.008 & 0.470 & 5.511 & 0.122 & 7.376 & 0.019 & 0.144 & 0.009 & 0.223 & 0.002 & 21.829 & 2.695 & 1493.761 & 19.283 & 2.038 & 0.044 & 6.306 & 0.085 \\
Br73 & 95.520 & -6.318 & 6497.806 & 279.208 & 9.128 & 0.176 & 1.343 & 0.562 & 13.314 & 0.380 & 15.805 & 0.440 & 0.086 & 0.006 & 1.304 & 0.085 & 15.779 & 2.348 & 3111.288 & 74.399 & 17.148 & 1.319 & 14.315 & 0.389 \\
Br75 & 102.248 & -23.995 & 6829.598 & 290.963 & 9.269 & 0.205 & 1.858 & 0.996 & 9.710 & 0.391 & 13.464 & 0.237 & 0.162 & 0.011 & 1.326 & 0.051 & 44.743 & 5.267 & 2496.357 & 65.916 & 21.093 & 0.989 & 11.141 & 0.334 \\
Br81 & 285.416 & -0.457 & 3468.979 & 46.229 & 8.352 & 0.207 & 0.225 & 0.112 & 5.535 & 0.063 & 6.293 & 0.087 & 0.064 & 0.003 & 0.159 & 0.002 & 4.108 & 0.453 & 1397.674 & 16.580 & 1.289 & 0.043 & 5.883 & 0.072 \\
Col197 & 131.215 & -41.260 & 924.127 & 1.751 & 6.605 & 0.109 & 0.004 & 0.000 & 8.204 & 0.251 & 8.447 & 0.207 & 0.021 & 0.013 & 0.043 & 0.001 & 0.584 & 1.206 & 1928.107 & 43.010 & 0.068 & 0.001 & 8.323 & 0.206 \\
Cz24 & 88.852 & 20.877 & 3722.727 & 90.968 & 9.080 & 0.180 & 1.203 & 0.502 & 9.280 & 0.027 & 11.969 & 0.117 & 0.126 & 0.005 & 0.346 & 0.019 & 25.298 & 2.297 & 2360.600 & 8.570 & 2.440 & 0.224 & 10.455 & 0.043 \\
Cz30 & 112.795 & -9.946 & 6108.557 & 169.368 & 9.033 & 0.189 & 1.081 & 0.487 & 10.157 & 0.145 & 13.328 & 0.173 & 0.135 & 0.001 & 0.493 & 0.015 & 31.485 & 0.724 & 2570.502 & 30.757 & 3.940 & 0.153 & 11.519 & 0.156 \\
ESO92\_05 & 150.789 & -64.754 & 11149.450 & 574.221 & 9.199 & 0.338 & 1.584 & 1.412 & 9.984 & 0.676 & 16.133 & 3.108 & 0.237 & 0.065 & 1.932 & 0.302 & 105.846 & 99.093 & 2693.215 & 242.282 & 30.886 & 2.077 & 12.147 & 1.243 \\
IC4665 & 266.532 & 5.634 & 343.345 & 0.239 & 7.514 & 0.230 & 0.032 & 0.017 & 7.383 & 0.089 & 7.922 & 0.007 & 0.035 & 0.006 & 0.129 & 0.002 & 1.464 & 0.529 & 1784.086 & 10.425 & 0.654 & 0.026 & 7.637 & 0.049 \\
M67 & 132.849 & 11.817 & 837.267 & 0.628 & 9.227 & 0.178 & 1.688 & 0.737 & 7.789 & 0.010 & 9.295 & 0.002 & 0.088 & 0.000 & 0.560 & 0.001 & 10.115 & 0.181 & 1946.596 & 1.085 & 8.009 & 0.037 & 8.412 & 0.005 \\
NGC2141 & 90.744 & 10.455 & 4052.221 & 34.795 & 9.262 & 0.154 & 1.831 & 0.707 & 11.710 & 0.046 & 12.967 & 0.096 & 0.050 & 0.005 & 0.410 & 0.004 & 4.671 & 0.963 & 2720.446 & 7.263 & 3.003 & 0.046 & 12.287 & 0.037 \\
NGC2158 & 91.859 & 24.097 & 3706.334 & 20.611 & 9.269 & 0.160 & 1.858 & 0.704 & 10.799 & 0.026 & 11.932 & 0.025 & 0.049 & 0.001 & 0.325 & 0.004 & 4.111 & 0.316 & 2531.236 & 2.864 & 2.213 & 0.046 & 11.319 & 0.014 \\
NGC2232 & 96.977 & -4.771 & 318.036 & 0.224 & 7.123 & 0.234 & 0.013 & 0.007 & 8.437 & 0.029 & 8.616 & 0.031 & 0.011 & 0.001 & 0.045 & 0.002 & 0.160 & 0.043 & 1969.963 & 5.964 & 0.073 & 0.006 & 8.525 & 0.028 \\
NGC2243 & 97.396 & -31.283 & 3928.227 & 23.567 & 9.439 & 0.167 & 2.748 & 1.115 & 10.445 & 0.019 & 16.863 & 0.124 & 0.234 & 0.002 & 1.838 & 0.022 & 109.860 & 2.952 & 2815.872 & 10.129 & 26.733 & 0.271 & 12.779 & 0.052 \\
NGC2244 & 97.985 & 4.926 & 1415.235 & 4.221 & 6.613 & 0.122 & 0.004 & 0.001 & 9.451 & 0.129 & 10.393 & 0.238 & 0.050 & 0.010 & 0.060 & 0.003 & 3.727 & 2.122 & 2251.631 & 30.092 & 0.103 & 0.014 & 9.910 & 0.150 \\
NGC2264 & 100.273 & 9.572 & 706.459 & 1.968 & 6.756 & 0.157 & 0.005 & 0.002 & 8.652 & 0.186 & 8.950 & 0.199 & 0.020 & 0.016 & 0.085 & 0.004 & 0.590 & 1.664 & 2023.196 & 26.543 & 0.253 & 0.019 & 8.783 & 0.129 \\
NGC2355 & 109.250 & 13.762 & 1751.095 & 5.018 & 9.232 & 0.171 & 1.706 & 0.674 & 9.754 & 0.110 & 10.906 & 0.176 & 0.057 & 0.007 & 0.599 & 0.033 & 5.286 & 1.676 & 2316.546 & 22.900 & 7.534 & 0.504 & 10.234 & 0.114 \\
NGC2420 & 114.602 & 21.574 & 2311.418 & 8.766 & 9.352 & 0.169 & 2.250 & 0.908 & 8.222 & 0.074 & 11.303 & 0.062 & 0.157 & 0.007 & 0.918 & 0.010 & 36.508 & 3.306 & 2153.989 & 5.499 & 14.210 & 0.151 & 9.425 & 0.027 \\
NGC2425 & 114.579 & -14.888 & 3094.027 & 21.859 & 9.295 & 0.160 & 1.975 & 0.729 & 8.202 & 0.050 & 11.593 & 0.032 & 0.171 & 0.002 & 0.490 & 0.008 & 43.723 & 1.177 & 2188.967 & 8.245 & 4.731 & 0.118 & 9.598 & 0.040 \\
NGC2451 & 116.176 & -37.942 & 367.535 & 0.148 & 7.440 & 0.223 & 0.027 & 0.015 & 8.305 & 0.001 & 8.857 & 0.094 & 0.032 & 0.005 & 0.063 & 0.001 & 1.369 & 0.464 & 1979.672 & 9.097 & 0.140 & 0.008 & 8.572 & 0.044 \\
NGC2516 & 119.521 & -60.792 & 407.088 & 0.089 & 8.097 & 0.269 & 0.125 & 0.089 & 7.310 & 0.021 & 8.183 & 0.000 & 0.056 & 0.001 & 0.095 & 0.000 & 3.861 & 0.198 & 1801.942 & 2.523 & 0.344 & 0.003 & 7.721 & 0.011 \\
NGC2547 & 122.533 & -49.194 & 382.382 & 0.179 & 7.336 & 0.259 & 0.021 & 0.014 & 8.190 & 0.011 & 8.764 & 0.127 & 0.033 & 0.006 & 0.053 & 0.002 & 1.501 & 0.626 & 1958.170 & 13.602 & 0.100 & 0.010 & 8.468 & 0.065 \\
NGC3532 & 166.393 & -58.693 & 471.884 & 0.109 & 8.376 & 0.249 & 0.237 & 0.155 & 7.988 & 0.020 & 8.062 & 0.001 & 0.004 & 0.001 & 0.121 & 0.000 & 0.025 & 0.014 & 1864.877 & 2.262 & 0.566 & 0.002 & 8.020 & 0.010 \\
NGC4815 & 194.507 & -64.959 & 3142.276 & 12.634 & 8.411 & 0.174 & 0.258 & 0.109 & 6.558 & 0.112 & 7.118 & 0.033 & 0.040 & 0.006 & 0.103 & 0.000 & 1.840 & 0.609 & 1608.696 & 16.518 & 0.480 & 0.007 & 6.824 & 0.075 \\
NGC6005 & 238.950 & -57.435 & 2388.113 & 9.511 & 8.933 & 0.171 & 0.857 & 0.339 & 4.935 & 0.070 & 6.374 & 0.007 & 0.127 & 0.007 & 0.115 & 0.000 & 15.206 & 1.619 & 1324.177 & 10.244 & 0.671 & 0.008 & 5.567 & 0.043 \\
NGC6067 & 243.295 & -54.231 & 1957.161 & 3.378 & 7.949 & 0.187 & 0.088 & 0.040 & 6.580 & 0.011 & 6.901 & 0.106 & 0.023 & 0.007 & 0.070 & 0.001 & 0.608 & 0.469 & 1589.522 & 10.960 & 0.236 & 0.005 & 6.737 & 0.049 \\
NGC6253 & 254.770 & -52.714 & 1606.201 & 3.190 & 9.267 & 0.167 & 1.852 & 0.779 & 5.335 & 0.016 & 6.849 & 0.007 & 0.124 & 0.000 & 0.216 & 0.001 & 15.333 & 0.222 & 1422.510 & 2.967 & 2.091 & 0.018 & 5.992 & 0.012 \\
NGC6259 & 255.192 & -44.676 & 2158.990 & 3.723 & 8.215 & 0.178 & 0.164 & 0.070 & 5.721 & 0.020 & 6.227 & 0.020 & 0.042 & 0.000 & 0.041 & 0.000 & 1.780 & 0.051 & 1416.017 & 4.592 & 0.090 & 0.001 & 5.963 & 0.020 \\
NGC6281 & 256.188 & -37.940 & 520.762 & 0.338 & 8.437 & 0.234 & 0.273 & 0.161 & 7.574 & 0.013 & 7.921 & 0.006 & 0.022 & 0.001 & 0.072 & 0.000 & 0.605 & 0.068 & 1806.311 & 0.859 & 0.207 & 0.001 & 7.742 & 0.004 \\
NGC6405 & 265.067 & -32.228 & 451.869 & 0.274 & 7.719 & 0.240 & 0.052 & 0.030 & 7.700 & 0.018 & 7.759 & 0.015 & 0.003 & 0.002 & 0.043 & 0.000 & 0.017 & 0.033 & 1803.377 & 0.657 & 0.077 & 0.001 & 7.728 & 0.003 \\
NGC6633 & 276.805 & 6.559 & 389.528 & 0.201 & 8.674 & 0.212 & 0.472 & 0.248 & 7.212 & 0.034 & 8.133 & 0.004 & 0.060 & 0.002 & 0.082 & 0.000 & 4.348 & 0.379 & 1785.875 & 3.570 & 0.260 & 0.000 & 7.646 & 0.016 \\
NGC6709 & 282.833 & 10.322 & 1048.055 & 1.571 & 8.207 & 0.210 & 0.161 & 0.088 & 7.030 & 0.155 & 7.561 & 0.009 & 0.036 & 0.011 & 0.146 & 0.002 & 1.515 & 1.030 & 1707.541 & 17.164 & 0.882 & 0.027 & 7.279 & 0.079 \\
NGC6802 & 292.646 & 20.258 & 2768.780 & 13.561 & 8.534 & 0.175 & 0.342 & 0.145 & 6.305 & 0.132 & 7.450 & 0.133 & 0.084 & 0.003 & 0.067 & 0.000 & 7.856 & 0.639 & 1610.858 & 29.043 & 0.193 & 0.001 & 6.834 & 0.132 \\
Pismis15 & 143.687 & -48.040 & 2254.343 & 10.105 & 8.652 & 0.182 & 0.448 & 0.201 & 7.215 & 0.159 & 8.421 & 0.005 & 0.077 & 0.010 & 0.140 & 0.000 & 7.289 & 1.983 & 1812.396 & 19.757 & 0.708 & 0.007 & 7.771 & 0.093 \\
Pismis18 & 204.226 & -62.091 & 2598.111 & 12.083 & 8.508 & 0.184 & 0.322 & 0.154 & 6.502 & 0.036 & 6.919 & 0.004 & 0.031 & 0.002 & 0.090 & 0.000 & 1.037 & 0.181 & 1581.745 & 4.387 & 0.385 & 0.007 & 6.701 & 0.019 \\
Rup134 & 268.175 & -29.534 & 2296.640 & 12.284 & 8.308 & 0.218 & 0.203 & 0.104 & 4.534 & 0.093 & 6.241 & 0.160 & 0.158 & 0.022 & 0.109 & 0.005 & 22.591 & 6.904 & 1252.751 & 3.717 & 0.631 & 0.038 & 5.265 & 0.015 \\
Trumpler14 & 161.264 & -59.696 & 2296.983 & 6.845 & 6.794 & 0.208 & 0.006 & 0.003 & 7.789 & 0.509 & 7.832 & 0.630 & 0.043 & 0.036 & 0.030 & 0.001 & 2.325 & 6.472 & 1820.377 & 102.753 & 0.037 & 0.005 & 7.809 & 0.486 \\
Trumpler20 & 189.887 & -60.632 & 3279.385 & 10.675 & 9.200 & 0.163 & 1.584 & 0.592 & 7.014 & 0.002 & 7.750 & 0.028 & 0.049 & 0.001 & 0.162 & 0.000 & 2.923 & 0.209 & 1724.141 & 3.025 & 1.040 & 0.005 & 7.356 & 0.014 \\
Trumpler23 & 240.213 & -53.537 & 2471.292 & 10.055 & 8.520 & 0.164 & 0.331 & 0.123 & 5.042 & 0.091 & 6.399 & 0.065 & 0.118 & 0.004 & 0.018 & 0.000 & 13.424 & 0.842 & 1343.303 & 19.057 & 0.017 & 0.001 & 5.649 & 0.081 \\
Trumpler5 & 99.127 & 9.458 & 2904.927 & 9.492 & 9.337 & 0.166 & 2.173 & 0.850 & 10.702 & 0.019 & 12.289 & 0.014 & 0.069 & 0.000 & 0.104 & 0.000 & 8.113 & 0.182 & 2556.112 & 2.946 & 0.242 & 0.001 & 11.445 & 0.015 \\
gamma2\_Vel & 122.374 & -47.353 & 346.884 & 0.166 & 6.971 & 0.225 & 0.009 & 0.004 & 8.248 & 0.074 & 8.338 & 0.140 & 0.008 & 0.007 & 0.067 & 0.004 & 0.088 & 0.307 & 1921.525 & 18.842 & 0.169 & 0.019 & 8.291 & 0.090 \\
lam\_Ori & 83.814 & 9.888 & 393.775 & 0.213 & 6.719 & 0.157 & 0.005 & 0.001 & 8.527 & 0.037 & 8.948 & 0.011 & 0.023 & 0.002 & 0.071 & 0.003 & 0.774 & 0.155 & 2012.117 & 4.313 & 0.175 & 0.017 & 8.729 & 0.020 \\
\end{longtable}

